Shorts vs. Regular Videos on YouTube: A Comparative Analysis of User Engagement and Content Creation Trends

YouTube introduced the Shorts video format in 2021, allowing users to upload short videos that are prominently displayed on its website and app. Despite having such a large visual footprint, there are no studies to date that have looked at the impact Shorts introduction had on the production and consumption of content on YouTube. This paper presents the first comparative analysis of YouTube Shorts versus regular videos with respect to user engagement (i.e., views, likes, and comments), content creation frequency and video categories. We collected a dataset containing information about 70k channels that posted at least one Short, and we analyzed the metadata of all the videos (9.9M Shorts and 6.9M regular videos) they uploaded between January 2021 and December 2022, spanning a two-year period including the introduction of Shorts. Our longitudinal analysis shows that content creators consistently increased the frequency of Shorts production over this period, especially for newly-created channels, which surpassed that of regular videos. We also observe that Shorts target mostly entertainment categories, while regular videos cover a wide variety of categories. In general, Shorts attract more views and likes per view than regular videos, but attract less comments per view. However, Shorts do not outperform regular videos in the education and political categories as much as they do in other categories. Our study contributes to understanding social media dynamics, to quantifying the spread of short-form content, and to motivating future research on its impact on society.

==> related_work.tex <==


% YOUTUBE RESEARCH
% TO READ
%https://dl.acm.org/doi/pdf/10.1145/3447535.3462512
%https://dl.acm.org/doi/pdf/10.1145/3485447.3512102?casa_token=oHyO2VP5S0oAAAAA:Cwr3LbA-5_xprD4u6tHY71UjnEga2JYsEcm7bDVtnhCXGmkCt_4eJaQdIbgU_k2VaJpSYUamrOA
%https://dl.acm.org/doi/pdf/10.1145/3394231.3397916?casa_token=tXwzfxmpACwAAAAA:Pp4V8HPqBNMilRauJZeI0SFXTLgw3UE3kBBQWBXCg51rHw7KSuXVNJKKnzGBLm82dL6KJfJkh9k
%https://dl.acm.org/doi/pdf/10.1145/3555601?casa_token=Q-1IpZFTPc4AAAAA:XqrKV8aO04ZF88_vPxMlEZwldjy6AhYbwKsLTf6LajHbLR_nwqNYLGiI4eQs6Y5gQUrUQ8l986Y

Our research delves into the dynamic shifts in content creation and user behavior resulting from evolving platform policies, with a special focus on YouTube Shorts, which is a popular instance of short-form video concept. We now provide a brief survey on existing research related to short-form videos and the effect of platform policies on user behavior. 

\subsection{Short-Form Videos}

YouTube is the primary video-oriented social media platform. Past studies on YouTube focused on its role on propagating disinformation~\cite{hussain2018analyzing, hussein_measuring_2020, papadamou_it_2022}, on video popularity~\cite{borghol_characterizing_2011, wattenhofer_youtube_2012}, on attention dynamics~\cite{lee_whose_2022}, and on user interactions~\cite{wu2021crosspartisan}. Nonetheless, it is unclear if the results of these analyses focusing on regular video content hold for short-form videos as the way people interact with these two types of videos are different. 

Short-form videos are currently understudied and large-scale analyses of such data are relatively uncommon. This is first because the short-form video concept has gained widespread popularity and became the primary feature of social media platforms only recently, e.g., YouTube introduced Shorts and their section in 2021. Second, the platforms have been restrictive in their data-sharing policies. YouTube announced its research API in 2022, TikTok announced it in 2023, and Instagram still does not allow large-scale analysis of Reels. As such, our work is one of the few that analyze short-form videos and the first to analyze YouTube Shorts to the best of our knowledge. We now survey the existing works on short-form videos, which mostly rely on TikTok as data source.

Past analyses of TikTok mainly focused on its trending and recommendation algorithm. Klug et al. studied the characteristics of trending videos on TikTok and found that they have high video engagements and are more likely to be posted at certain times~\cite{klug2021trick}. They also report that using trending hashtags do not necessarily contribute to a video being trending. Simpson et al. investigated the impact of TikTok's algorithm on LGBTQ+ users and highlighted algorithmic exclusion and resilience in identity work~\cite{simpson2021you}. Boeker and Urman studied TikTok's recommendation algorithm and reported that it is influenced by users' location, language, and engagement with the content~\cite{boeker2022empirical}. Lee et al. employed a qualitative method in which they interview TikTok users to understand how they perceive and interact with TikTok's algorithms~\cite{lee2022algorithmic}. Other studies focused on how the platform shapes political communication by analyzing users' sentiment against the politicians~\cite{zeng2021okboomer}, hyperpartisan activity~\cite{medina2020dancing}, and the platforms' policies against misinformation~\cite{ling2023learn}.

\subsection{Impact of Platform Policies on Users}

Popular social media platforms introduce new policies from time to time. This may be due to external actors (e.g., governments) enforcing platforms to adopt new policies such as censorship~\cite{elmas2021dataset}, privacy policies~\cite{liu2021have}, and moderate hate speech~\cite{kozyreva2023resolving} and disinformation~\cite{papakyriakopoulos2022impact}. In other cases, platforms themselves may introduce changes to the platforms to enhance user experience. In all cases, such changes encourage users to change their behavior and adapt, which eventually shapes public communication. Such behavioral change may manifest itself in user content. For instance, users tend to use more abbreviations and contracted forms when they are constrained by the length of their content, but they also tend to create content with better quality~\cite{gligoric2018constraints}. They may also game platforms' policies to manipulate social media, such as purchasing popular accounts instead of growing new accounts~\cite{elmas2023misleading} or maintaining backup accounts to recover from platform suspensions~\cite{merhi2023information}. Other actors such as researchers may also be affected by platforms' data collection policies such as denying access to removed content~\cite{elmas2023impact} or limiting access to the API~\cite{braun2023journalism}. In this work, we study the impact of the introduction of Shorts on channel behavior by comparing the channels' regular videos and Shorts, which have not been studied to date. 



